Formulation of Relativistic Dissipative Spin Hydrodynamics

The primary objective of this thesis is to develop a consistent theoretical framework of dissipative hydrodynamics for a relativistic fluid with spin - hereafter referred to as relativistic dissipative spin hydrodynamics. In this framework, the dynamical description of a relativistic fluid requires a new macroscopic variable, the spin density, which is associated with a spin tensor. This tensor, defined as the expectation value of a rank-3 tensor operator in quantum field theory, contributes to the system's total angular momentum. The need for such a theory is motivated by recent measurements of spin polarization of hadrons produced in non-central relativistic heavy-ion collisions. Two distinct formulation methods are employed. The first is grounded in covariant thermodynamics and extends the conventional Navier-Stokes and M\"uller-Israel-Stewart theories of relativistic hydrodynamics by incorporating a spin tensor. The second is based on principles of relativistic quantum statistical mechanics, building upon and generalizing the foundational Zubarev approach. Both formulations aim to construct a closed system of evolution equations for the macroscopic variables and, via an entropy-current analysis, to identify the dissipative currents and their associated transport coefficients. These two approaches provide different perspectives for future applications focused on spin polarization measurements. Beyond its phenomenological relevance, the theory also opens several avenues for further theoretical developments. These include the verification of the thermodynamic relations employed in the first formulation method using microscopic frameworks, as well as a deeper understanding of the emerging transport coefficients - particularly those associated with the spin tensor - through microscopic modeling or data-driven parameter extraction.

==> mitthesis-defaultfonts.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-defaultfonts.tex}[2023/09/12 v1.03 Load Computer/Latin Modern text and math fonts]

%% Default fonts
%
\ifpdftex
	\typeout{^^JLoading Computer Modern text and math fonts (default for pdftex).^^J}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\typeout{^^JLoading Latin Modern text and math fonts (default for unicode engines).^^J}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi


==> mitthesis-fira-newtxsf.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-fira-newtxsf.tex}[2023/09/12 v1.04 Load Fira Sans text font with newtx sans serif math font and Inconsolata typewriter font]

%% Fira Sans text font with newtx sans serif math font and Inconsolata typewriter font
%
\ifpdftex
	\typeout{^^JLoading Fira sans text font with newtx sans serif math font and Inconsolata typewriter^^J}
    \RequirePackage[sfdefault,scaled=0.90]{FiraSans} % sans serif text package %,scaled=.85
	\RequirePackage[T1]{fontenc}
    \RequirePackage[varqu,varl,scaled=1.05]{zi4} % inconsolata font for typewriter
    \RequirePackage[scaled=1.05]{newtxsf} % sans serif math
 	\RequirePackage{bm}
\else
	\ClassWarning{mitnewthesis}{The fira-newtxsf font set requires pdflatex. Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi


==> mitthesis-heros-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-heros-stix2.tex}[2023/09/12 v1.02 Load TeX Gyre Heros (sans serif) text font with STIX Two Math font and Inconsolata monospaced font]

%% TeX Gyre Heros (sans serif) text font with STIX Two Math font and Inconsolata monospaced font
%
% These fonts are available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The heros-stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\typeout{^^JTeX Gyre Heros (sans serif) text font with STIX2 math font and Inconsolata monospaced font.^^J}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package

    \setmainfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,
	]        
    \setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,
	]        
   \setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package and is in CTAN https://ctan.org/tex-archive/fonts/inconsolata
        Scale=1.05,
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02,+ss03},
    ]             
    \setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed %% https://github.com/stipub/stixfonts
    	Scale=MatchUppercase,
    	Extension = .otf,
		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
    ]
    % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
    %    
    \setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Heros bold, https://github.com/stipub/stixfonts
    \setmathfontface\mathit{STIXTwoText-Italic.otf}[]
    \setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX Two
     %         
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> mitthesis-libertine.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-libertine.tex}[2023/09/12 v1.02 Load Libertine and related fonts]

%% Linux Libertine (serif) text font with newtxmath[libertine] (pdftex) or Libertinus (unicode) math font
%
%  These fonts are available here https://ctan.org/tex-archive/fonts/libertine/opentype 
%						 and here https://github.com/alerque/libertinus
% install these as system fonts on your computer
%
\ifpdftex
	\typeout{^^JLoading newtx-libertine text and math fonts with Insolata typewriter font^^J}
    \RequirePackage[lining,semibold]{libertine} 
    \RequirePackage[T1]{fontenc}
    \RequirePackage[varqu,varl]{inconsolata}% typewriter
%    \usepackage{amsthm}% must be loaded before newtxmath
    \RequirePackage[libertine,vvarbb]{newtxmath}
    \RequirePackage{bm}% load after all math to give access to bold math
\else
	\typeout{^^JLoading Linux Libertine (serif) text font with Libertinus math font^^J}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode math loads the fontspec package
 	%
    \setmainfont{LinLibertine}[% Linux Libertine O  
    	Extension = .otf,
    	UprightFont = *_R,
    	ItalicFont = *_RI,
    	BoldFont = *_RZ, % Libertine O Semibold
    	BoldItalicFont = *_RZI, % Libertine O Semibold Italic
    %	Ligatures=Rare,% TeX
    %	Numbers=OldStyle,%
    	RawFeature={+ss05},% +ss02 would change J, K, R; +ss05 changes W	
        ]    
    \setmonofont{LinLibertine}[% Linux Libertine Mono O
    	Scale=0.9,
	    Extension = .otf,
    	UprightFont = *_M,
    	ItalicFont = *_MO,% oblique
    	BoldFont = *_MB,
	    BoldItalicFont = *_MBO,% oblique
	]    
    \setsansfont{LinBiolinum}[% Linux Biolinum O
    	Extension = .otf,
    	UprightFont = *_R,
    	ItalicFont = *_RI,
    	BoldFont = *_RB,
	    BoldItalicFont = *_RBO,% oblique
    	Scale=MatchUppercase]
	%    	
    %% a Libertine-style math font
    \setmathfont{libertinusmath-regular}[%
     	Extension = .otf,   
    	Scale=MatchUppercase,
		BoldFont = *,% This font lacks a bold version
    	RawFeature={+ss08},% +ss08 gives slanted integrals (no other features) 	
    	]
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2}   
\fi


==> mitthesis-lucida.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-lucida.tex}[2023/09/12 v1.02 Load Lucida fonts]

%% Lucida Bright and Lucida Bright Math fonts (available from the TeX Users Group)

\typeout{^^JLucida Bright and Lucida Bright Math fonts^^J}

\ifpdftex
	\RequirePackage[LY1]{fontenc}
	\RequirePackage[expert,vargreek,altbullet,seriftt]{lucidabr}   % switch text and math fonts
	\RequirePackage{bm}
\else
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package

    % FEATURE 	DESCRIPTION 											DEFAULT
    % dlig 		discretionary ligatures (f-ligatures in typewriter fnt) off
    % liga 		standard ligatures (f-ligatures, not monospaced fonts) 	on
    % onum 		old style numbers (Lucida Bright only)					off
    % smcp 		small caps 	(Lucida Bright, upright only)				off
    % zero 		slashed zero (sans and monospaced fonts)				off
    % locl 		script/language specific (localized) forms 				on
    %
    % FEATURE 	FONT 						DESCRIPTION
    % ss01 		Lucida Sans & Typewriter 	use dotted zero: 𝟶 vs. default 0.
    % ss01 		use Lucida-standard shapes:
    % 			Lucida Grande Mono 			ØOQ vs. default 0OQ;
    % 			Lucida Console 				ØOQ vs. default 0OQ.
    
    \setmainfont{LucidaBrightOT}[% main rm
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Italic,
          BoldFont=*-Demi,
    	  BoldItalicFont=*-DemiItalic,
          BoldItalicFeatures={Color=Purple4},
    %     UprightFeatures={Color=Salmon3},
    	  Scale=0.92,
    %	  Numbers ={OldStyle}, 
      ]
    %
    \setsansfont{LucidaSansOT}[% main sans
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Italic,
          BoldFont=*-Demi,
    	  BoldItalicFont=*-DemiItalic,
    	  Scale=MatchUppercase,
      ]
    %
    \setmonofont{LucidaSansTypewriterOT}[% main typewriter
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Oblique,
          BoldFont=*-Bold,
          BoldItalicFont=*-BoldOblique,
      	  Scale=MatchUppercase,
      ]
    
    %% MATH FONTS
    %
    % ss01 	alternate Latin lower case math italic identical to text italic. This option is not recommended as Greek 𝜈 (nu) and Latin 𝑣 (vee) become too similar
    % ss02 	smaller arrows (original Type 1 size): ⇑ vs. default ⇑.
    % ss03 	attempt to imitate Type 1 fonts
    % ss04 	calligraphic alternative (similar to the Type 1 design) to the math script alphabet
    % ss05 	use a slashed-zero style for the empty set character (U+2205): Ø vs. default ∅
    % ss08 	emphasize right and bottom edges of the d’Alembertian operator (U+29E0, \laplac), to follow the design of the Laplace operator (U+2206, \increment, Δ); the default design emphasizes the left and upper edges. Also available in the bold math font.
    %
    \setmathfont{LucidaBrightMathOT}[% main math
    	  Scale=MatchUppercase,
    	  Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,
%    	  BoldFeatures={Color=Chartreuse4},
    	  RawFeature ={+ss04,+ss08}, %
    ]
 
%% LucidaMath-OT contains a *serif* typerwriter font. If you prefer a sans serif typerwriter font, you can use the following two settings. 
% 
%    \setmathfont{LucidaSansTypewriterOT}[% <== NB: setting a text font where math font should go.
%    	  Scale=MatchUppercase,
%          range=tt,
%    	  Color=NavyBlue,
%          Extension=.otf,
%          script-features = {},     
%          sscript-features = {},     
%    	  BoldFont=LucidaSansTypewriterOT-Bold.otf,
%    	  BoldFeatures={Color=Salmon3},
%    ]
%    %
%    \setmathfontface\mathtt{LucidaSansTypewriterOT-Bold}[% bold upright typewriter font in boldmath.
%    	  version=bold,
%    	  Scale=MatchUppercase,
%          Extension=.otf,    
%    ]
	%
    \setmathfont{LucidaBrightMathOT}[%
    	  range={scr},% to make scr differ from cal
    	  RawFeature={-ss04},
    	  Scale=MatchUppercase,
          Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,% could be overridden by bold separate version
    ]
    \setmathfont{LucidaBrightMathOT}[% -Demi .. sufficient this way, since bold set above.
    	  range={bfscr},% need to call \symbfscr manually - bug in unicode-math version & range interaction
    	  RawFeature={-ss04},
    	  Scale=MatchUppercase,
          Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,
    ]
    %% Fix unicode-math operator font not set up for bold face (default \mathrm). See https://github.com/wspr/unicode-math/issues/468
    \setoperatorfont\normalfont
    %
    % note \mathbfit = \symbfit
    
    % The specialized one-off Lucida fonts:
    \newfontface\LucidaBlackletter{LucidaBlackletterOT}[%
    	Scale=0.95,% <== NB
    	Extension=.otf,
    	]
    \newfontface\LucidaCalligraphy{LucidaCalligraphyOT}[%
    	Scale=MatchUppercase,
    	Extension=.otf,
    	]
    \newfontface\LucidaHandwriting{LucidaHandwritingOT}[%
    	Scale=MatchUppercase,
    	Extension=.otf,
     	]
    % GrandeMono and Console fonts:
    \newfontface\LucidaGrandeMonoDK{LucidaGrandeMonoDK}[%	
    	Scale=MatchUppercase,
    	Extension=.otf,
        UprightFont=*,
        ItalicFont=*-Italic,
        BoldFont=*-Bold,
        BoldItalicFont=*-BoldItalic,
    	]
    \newfontface\LucidaConsole{LucidaConsoleDK}[%
    	Scale=MatchLowercase,% <=== NB
    	Extension=.otf,
        UprightFont=*,
        ItalicFont=*-Italic,
        BoldFont=*-Bold,
        BoldItalicFont=*-BoldItalic,
    	]
\fi


==> mitthesis-newtx-sans-text.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-newtx-sans-text.tex}[2023/10/03 v1.03 Load newtx sans-serif text and regular math fonts]

%% newtx package with sans-serif text (Helvetica-like text with Times-like math)
%
\ifpdftex
	\RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91,defaultsups]{newtx}% upint for upright integrals
	\AtEndPreamble{% added to accommodate v1.731 of newtx, 2023/11/03
	    \renewcommand{\familydefault}{\sfdefault}% use sans for main text
%	    \renewcommand{\rmdefault}{\sfdefault}% uses sans for \textrm{}, if that's desired.
	}
%   these two commands enable hyphenation of the typewriter font - https://tex.stackexchange.com/a/204421/119566
%    \input{t1ntxtt.fd}
%    \DeclareFontFamily{\encodingdefault}{\ttdefault}{\hyphenchar\font=`\-} % 
	\RequirePackage{bm}% bold math
\else
	\ClassWarning{mitnewthesis}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi

	

==> mitthesis-newtx.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-newtx.tex}[2023/09/12 v1.03 Load newtx text and math fonts]

\ifpdftex
	\typeout{^^JLoading newtx fonts with inconsolata typewriter^^J}
	\RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91]{newtx}% stix2, upint
    \RequirePackage[varl,varqu,hyphenate,mono]{inconsolata}% sans typewriter font; mono = fixed word spacing, hyphenate = allow hyphenation 
	\RequirePackage{bm}
	\let\textsuperscript\textsu% newtx changes the default superiors font; this is needed to get commas aligned in sequential footnotes
\else
	\ClassWarning{mitnewthesis}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi

	

==> mitthesis-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-stix2.tex}[2023/09/12 v1.03 Load STIX Two text and math fonts]

%% STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font
%
% These fonts are available at: 
%				https://github.com/stipub/stixfonts 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\typeout{^^JLoading STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font.^^J}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{STIXTwoText}[% Presumes these are system fonts! 
       	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
	]
	\setsansfont{texgyreheros}[% Presumes these are system fonts! 
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% 
	]        
	\setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package (it's in TeX Live)
        Scale=1.05,%
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02,+ss03},
    ]             
	\setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed
    	Scale=MatchUppercase,
    	Extension = .otf,
		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
   ]
   % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
   %
   \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> mitthesis-termes-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-termes-stix2.tex}[2023/09/12 v1.03 Load TeX Gyre Termes text font with STIX2 math font, Heros sans serif font, and Inconsolata monospaced font]

%% TeX Gyre Termes text font and Heros sans serif font with STIX2 math font and Inconsolata monospaced font
%
% These fonts are available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
% Install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The termes-stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\typeout{^^JLoading TeX Gyre Termes text font with STIX2 math font, Heros sans serif font, and Inconsolata monospaced font.^^J}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{TeXGyreTermesX}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},%% This stretch matches newtxtext a little better. 1.4
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
	\setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% same as for newtx; former value 0.9 too small 2022/01/15
	]        
	\setmonofont{Inconsolatazi4}[% This otf font ships with the LaTeX Inconsolata package (it's in TeX Live)
        Scale=1.05,% rescaled from 1, 22/03/10
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02,+ss03},
    ]             
	\setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes needed %% https://github.com/stipub/stixfonts
    	Scale=MatchUppercase,
    	Extension = .otf,
		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
   ]
   % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
   %
   \setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Termes bold, https://github.com/stipub/stixfonts
   \setmathfontface\mathit{STIXTwoText-Italic.otf}[]
   \setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX, not Termes
    %      
   \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> mitthesis-termes.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-termes.tex}[2023/09/12 v1.03 Load TeX Gyre Termes text and math fonts, Heros sans serif font, and Cursor monospaced font]

%% TeX Gyre Termes (Times-like) text font with Termes math font and Heros sans serif font and Cursor monospaced font
%
% These fonts are available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
% install these as system fonts on your computer
%
\ifpdftex
	\ClassWarning{mitnewthesis}{The termes fontset requires a unicode engine. Defaulting to CMR fonts.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\typeout{^^JLoading TeX Gyre Termes text and math fonts, Heros sans serif font, and Cursor monospaced font^^J}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress tiresome warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{TeXGyreTermesX}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
    \setsansfont{texgyreheros}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% same as for newtx; former value 0.9 too small 2022/01/15
	]        
   \setmonofont{texgyrecursor}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
        Scale=0.97,
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Italic,
        BoldFont = *-Bold, 
    	BoldItalicFont = *-BoldItalic,
%		BoldFeatures = { Color = VioletRed3 },
    ]             
    \setmathfont{texgyretermes-math}[% Presumes these are system fonts! Available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
    	Scale=MatchUppercase,
    	Extension = .otf,
		BoldFont = *, % termes-math does not have a bold version
%       Color=Red3, 
    ]
    %   
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2}
\fi


==> mydesign.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mydesign.tex}[2024/06/28 v1.04 Typographic design options for thesis]

%%%%%%%%%%  Color support  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Color package: xcolor. 
%% Change this if you prefer something else

\usepackage[dvipsnames,svgnames,x11names]{xcolor}

%% can add option [table] to xcolor to use color in tables (see xcolor documentation)


%%%%%%%%%%  Hyperlink and line number colors  %%%%%%%%%%%%%%

\AtBeginDocument{
    % Using color names from xcolor package
    \hypersetup{
    	linkcolor=Blue3,
    	citecolor=Blue3,
    	urlcolor=violet,
    	filecolor=red, 
    %	anchorcolor=yellow,%  not all pdf viewers recognize this field (although Firefox does): hyperref issues a warning
    %	colorscheme=phelype,% overrides link, cite, url, file colors with a preset scheme, through \DocumentMetadata
    	}
    %
    \ifmit@lineno
	    \renewcommand{\linenumberfont}{\sffamily\mdseries\tiny\color{violet}}% line numbers will be sans-serif, medium weight, tiny, and violet
	\fi
}

%%%%%%%%%  Caption support  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% see documentation for details of how to customize captions

\RequirePackage{caption}
\RequirePackage{subcaption}


%%%%%%%%%  Customize list environments  %%%%%%%%%%%%%%%%%%%%
% 
% see documentation for details of how to customize lists

%\RequirePackage{enumitem}


%%%%%%%%%  Customize titles and section headings  %%%%%%%%%%
% 
% see documentation for details of how to customize headings

\RequirePackage{titlesec}

% these titlesec commands just automate the bold math in some headings (rest follows default styles)
\titleformat{\section}{\mathversion{bold}\normalfont\Large\bfseries}{\thesection }{1em}{}
\titleformat{\subsection}{\mathversion{bold}\normalfont\large\bfseries}{\thesubsection}{1em}{}
\titleformat{\subsubsection}{\mathversion{bold}\normalfont\normalsize\bfseries}{\thesubsubsection}{1em}{}

% ==> NOT every font includes a bold math version, so you may need other math macros in the headings to get bold math <==


%%%%%%%%%  Change page margins  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% The default thesis margin is 1 inch all around. You may want different margins (e.g., to add a gutter for binding),
% in which case you can use the \newgeometry command from the geometry package.  Refer to the package documentation
% for details.
%
% mitthesis defaults: [top=1in,bottom=1in,left=1in,right=1in,marginparwidth=50pt,headsep=12pt,footskip=0.5in]
%
% The following tells the geometry package to use a two-sided layout with a 1 cm binding offset on the inside 
% 	and 1 inch margins all around, reducing textwidth slightly (by 0.7 cm). See geometry documentation, Section 8.2.
%
%\newgeometry{twoside, bindingoffset=1cm,margin=1in,marginparwidth=50pt,headsep=12pt,footskip=0.5in}

